Exact Imaging of Extended Targets Using Multistatic Interferometric Measurements

In this paper, we present a novel approach that can exactly recover extended targets in wave-based multistatic interferometric imaging, based on Generalized Wirtinger Flow (GWF) theory [1]. Interferometric imaging is a generalization of phase retrieval, which arises from cross-correlation of measurements from pairs of receivers in multistatic configuration. Unlike standard Wirtinger Flow, GWF theory guarantees exact recovery for arbitrary lifted forward models that satisfy the restricted isometry property over rank-1, positive semi-definite (PSD) matrices with a sufficiently small restricted isometry constant (RIC). To this end, we design a deterministic, lifted forward model for interferometric multistatic radar satisfying the exact recovery conditions of the GWF theory. Our results quantify a lower limit on the pixel spacing and the minimal sample complexity for exact multistatic radar imaging via GWF. We provide a numerical study of our RIC and pixel spacing bounds, which shows that GWF can achieve exact recovery with super-resolution. While our primary interest lies in radar imaging, our method is also applicable to other multistatic wave-based imaging problems such as those arising in acoustics and geophysics.

==> Signal_Model_v4_nored.tex <==
\section{Signal Model}\label{sec:signal}
% Suppose we have $N$ receivers each located at different spatial locations $\a_i^r$ and single
% transmitter located at $\a_i^t$. The data model for distributed multistatic
% passive radar is derived by correlating data from pair of receive antennas.
% Received data model can be expressed as

% \begin{table*}[!htbp]
% \caption{Table of Notations} % title of Table
% \centering % used for centering table
% {
% \small
% \begin{tabular}{p{1.3in}p{3.8in}}%p{0.1in}p{0.7in}p{1.4in}}

%   \hline \hline
%   Symbol & Description \\ % & &Symbol & Designation\\ [0.5ex] % inserts table
%   % heading
%   \hline % inserts single horizontal line
%   % $\omega$ & Frenquency
%   $M$ & Number of frequency samples \\
%   $N$ & Number of receivers \\
%   $K$ & Number of unknowns \\
%   $ d_{i,j}$ & Interferometric data from correlating receivers $i$ and $j$ \\
%   $\omega_c$, $\lambda_c$ & Center frequency and corresponding wavelength\\
%   $B$ & Bandwidth of the transmitted waveform\\
%   $\mathbf{x}$ & Spatial location in $\mathbb{R}^3$\\
%   $\bm{x}$ & Spatial location in $\mathbb{R}^2$\\
%   $\mathbf{a}^r_i$ & Location of $i$-th receiver in $\mathbb{R}^3$\\
%   $\mathbf{a}^t$ & Transmitter location in $\mathbb{R}^3$\\
%   $A_i$ & Amplitude function\\
%   $\phi_i$ & Bistatic phase function\\
%   $\varphi_{i,j}$ & Phase function in the lifted domain\\
%   $\rho$ & Reflectivity function\\
%   $\tilde{\rho}$ & Lifted Kronecker reflectivity\\
%   $\bm{\rho}$ & Discretized reflectivity in $\mathbb{R}^K$\\
%   $\tilde{\bm{\rho}}$ & Discretized Kronecker reflectivity in $\mathbb{R}^{K\times K}$\\
%   $\mathbf{L}_i^m$ & $m$-th measurement vector of the $i$-th receiver \\
% % $\brho$ & Scene of interest in $\mathbb{C}^N$ \\
% % $\mathbf{X}$ & Variable in the lifted domain in $\mathbb{C}^{N \times N}$ \\
% % $\tilde{\brho}$ & Kronecker scene $\brho \brho^H$ \\
% % $\mathit{P}$ & Global solution set with $\mathit{P}_{\brho_t} = \mathit{P}$ \\
%   $\mathcal{F}$, $\mathcal{F}^{\dagger}$ & Lifted forward model and its adjoint\\
% % $\mathcal{F}^H$ & Adjoint of $\mathcal{F}$/ Backprojection operator \\
%   $\mathcal{J}$ & Objective function of GWF\\
%   % $\nabla \mathcal{J}$ & Gradient of the objective function on the signal domain \\
% % $\mathrm{dist}$ & Distance metric \\
%   $\tilde{\mathbf{Q}}$ & Spectral matrix\\
%   % $\brho_0$ &  Initialization from spectral method \\
%   % $\tilde{\brho}_0$ & Initial lifted signal \\
%   % $\lambda_0, \mathbf{v}_0$  & Leading eigenvalue-eigenvector pair of $\tilde{\mathbf{Q}}$\\
%   $L$ & Side length of a square scene \\
%   $A$ & Arc length of imaging aperture\\
%   $\mathcal{K}$ & Kernel of $\mathcal{F}^{\dagger}\mathcal{F}$\\ %operator $\mathcal{F}$\\
%   $\Phi_{i,j}^{k,k',l,l'}$ & Phase function for $\mathcal{K}$\\
%   $\Delta_{res}$ & Fourier transform based range resolution\\
%   $\Delta$ & Pixel resolution/spacing\\
%   \hline \hline
% %\br %inserts single line
%   \end{tabular}}
%   %\end{indented}
%   \label{table:notation}
% \end{table*}

\subsection{Received Data Model}\label{subsec:signal1}
% In multistatic passive radar, we deploy several receivers around the scene of interest and receive
% signal scattered from the scene from at
% least one source of opportunity.
% The general multistatic passive radar scenario is illustrated in Fig.~\ref{fig:config}
% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=4in]{config_mult}
%   \caption{Typical multistatic passive radar scenario.}\label{fig:config}
% \end{figure}
Let $N$ be the number of receivers each deployed at different spatial locations $\a_i^r$,
$i=1,\dots,N$, % $\a_i^r\neq
% \a_j^r$, $i\neq j$
where subscript $i$ denotes the $i$-th receiver % (similarly for subscript $j$)
and superscript $r$ denotes receiver.  Assume a
single transmitter located at $\a^t$.
Furthermore, without loss of generality, we assume that the ground topography is flat.
% is represented by the function
  % $\psi:\mathbb{R}^2\rightarrow\mathbb{R}$.
Thus, each spatial location in three-dimensional space is represented as $\x=[\bm{x}, 0]$ where $\bm{x}\in\mathbb{R}^2$.
% We further assume that the scatterers and the
% transmit and receive antennas are all modeled as point source and sink without consideration to
% polarization or anisotropy.
Under these assumptions and that only the scattered field is being measured under the Born approximation, the received signal at each receiver for multistatic radar can be
modeled as ~\cite{cheney2009fundamentals}
% Furthermore, each receiver is equipped with pair
% of orthogonally polarized dipole antennas.  We approximate the targets as dipoles and derive the
% received signal model as~\cite{}
% \begin{equation}
%   % d_{i,j}(\omega) = \int_{D\times D}
%   % \mrm{e}^{\mrm{i}\omega/c_0\varphi_{i,j}(\x,\x')}A_{i,j}(\x,\x')\abs{\hat{s}(\omega)}^2
%   % \tilde{\rho}(\x,\x') d\bm{x} d\bm{x}'\label{eq:dij}
%   % d_{
%   d_i(\omega) = \int_D \mrm{e}^{\mrm{i}\omega/c_0 \phi_i(\x)}A_i(\x)\hat{s}(\omega)\rho(\x) d\x\label{eq:di}
% \end{equation}
% where $\bm{d}_i = [d_{i,H}, d_{i,V}]^T$ is a $2\times 1$ complex vector,
\begin{align}
  % d_{i,j}(\omega) = \int_{D\times D}
  % \mrm{e}^{\mrm{i}\omega/c_0\varphi_{i,j}(\x,\x')}A_{i,j}(\x,\x')\abs{\hat{s}(\omega)}^2
  % \tilde{\rho}(\x,\x') d\bm{x} d\bm{x}'\label{eq:dij}
  % d_{
  d_i(\omega) = &\int_{D} \mrm{e}^{\mrm{i}\omega/c_0
    \phi_i(\x)}A_i(\bm{x},\omega)\rho(\bm{x}) d\bm{x},\label{eq:di2}\\
  &\omega\in[\omega_c-B/2, \omega_c+B/2]\subset \mathbb{R}\nonumber
\end{align}
where
\begin{equation}
  \phi_i(\x) = \abs{\x-\a_i^r} + \abs{\x-\a^t}\label{eq:phi__}
  % \varphi_{i,j}(\x,\x') = \abs{\x-\a_i^r}+\abs{\x-\a^t}-\abs{\x'-\a_j^r}-\abs{\x'-\a^t}\label{eq:varphi}
\end{equation}
is the bistatic phase function, $D\subset\mathbb{R}^2$ is the support of the scene,
% $\tilde{D} = \{\bm{x} | \x\in
% D, \x=[\bm{x}, \psi(\bm{x})]^T\}$ is the scene of interest,
% and $A_{i}$ is antenna related terms (geometric spreading
% factor, antenna beampatterns, etc), and
$\omega$ is the fast-time frequency variable,
$\omega_c$ is the center frequency, $B$ is the bandwidth,
$c_0$ is the speed of light, $\rho$ is the target/scene reflectivity function; %which is assumed to be constant over the frequency band; 
and $A_i$ is the amplitude function given by
% Furthermore,
% in~\eqref{eq:di2}, we have assumed that
% and $\R(\x)$ is a
% The $\tilde{\rho}$ is the lifted target reflectivity function
% and is defined as the Kronecker product of the target reflectivity, denoted $\rho$ with itself,
% i.e. $\tilde{\rho} =  \rho\otimes\rho^*$.
% Assuming free-space background model along with isotropic assumption, the amplitude term $A_i$ can be modeled as%~\cite{}
\begin{equation}
  % A_{i,j}(\x,\x') \propto
  % \frac{J_i(\bm{x})J_j^*(\bm{x}')}{\abs{\x-\a_i^r}\abs{\x'-\a_j^r}\abs{\x-\a^t}\abs{\x'-\a^t}}\label{eq:Aij}
  A_i(\x,\omega) = \frac{J_i(\x,\omega)}{\abs{\x-\a_i^r}\abs{\x-\a^t}}%\approx
  % \frac{C}{\abs{\x-\a_i^r}\abs{\x-\a^t}}
  \label{eq:Aij}
\end{equation}
% where
with $J_i$ % is the term modeling
being the antenna beampattern. 
% The frequency $\omega$ ranges from $\omega_c-B/2$
% to $\omega_c+B/2$ where $\omega_c$ is the center frequency and $B$ is the bandwidth.

% \begin{assumption}\label{assump:gtop}
%   We assume that the ground topography is known and is represented by the function
%   $\psi:\mathbb{R}^2\rightarrow\mathbb{R}$.  Therefore, $\x=[\bm{x}, \psi(\bm{x})]$, where $\bm{x}\in\mathbb{R}^2$.
% \end{assumption}
% By~\assref{assump:gtop}, we can rewrite~\eqref{eq:di} as
% \begin{equation}
%   % d_{i,j}(\omega) = \int_{D\times D}
%   % \mrm{e}^{\mrm{i}\omega/c_0\varphi_{i,j}(\x,\x')}A_{i,j}(\x,\x')\abs{\hat{s}(\omega)}^2
%   % \tilde{\rho}(\x,\x') d\bm{x} d\bm{x}'\label{eq:dij}
%   % d_{
%   d_i(\omega) = \int_{\tilde{D}} \mrm{e}^{\mrm{i}\omega/c_0 \phi_i(\x)}A_i(\bm{x})\hat{s}(\omega)\rho(\bm{x}) d\bm{x}\label{eq:di2}
% \end{equation}
% where we make a slight abuse of notation and redefine $A_i$ and $\rho$ as function of $\bm{x}$ and
% \begin{equation}
%   \tilde{D} = \{\bm{x} | \x\in D, \x=[\bm{x}, \psi(\bm{x})]^T\}
% \end{equation}
% \subsection{Correlated Measurements}\label{subsec:signal2}
% % Given the data model~\eqref{eq:di2}, in passive radar, we typically cross-correlate the
% % measurements at pair of different receivers in order to reconstruct $\rho$.
% Given the data model~\eqref{eq:di2}, we consider the interferometric data, i.e. fast-time
% cross-correlation of the measurements at pairs of different receivers. %in order to reconstruct $\rho$.
% % \begin{assumption}\label{assump:1}
% Furthermore, we make the assumption that $\abs{J(\x,\omega_m)}=C$. In other words, we assume that the
% transmitted waveform has a flat spectrum.  This is typical of waveforms of opportunity such as
% phase shift keying (PSK) modulation found in orthogonal frequency-division multiplexing (OFDM)
% common among digital communications or typical radar waveforms.
% % In active radar, we have control  over the waveform design
% % and thus the assumption can be made valid.
% % \end{assumption}
% % These measurements are
% % generally called interferometric measurements and can be modeled as
% Using~\eqref{eq:di2}
\subsection{Correlated Measurements}\label{subsec:signal2}
% Given the data model~\eqref{eq:di2}, in passive radar, we typically cross-correlate the
% measurements at pair of different receivers in order to reconstruct $\rho$.
Given the data model~\eqref{eq:di2}, we consider the interferometric data, i.e. fast-time
cross-correlation of the measurements at pairs of different receivers. %in order to reconstruct $\rho$.
% \begin{assumption}\label{assump:1}
%We make the assumption the transmitted waveform has a flat spectrum. 
Furthermore, we make the assumption that $\abs{J_i(\x,\omega_m)} \approx C_i \in \mathbb{R}^{+}$. 
In other words, we assume %that we have isotropic receiver antennas, and 
that the
transmitted waveform has a flat spectrum, and that the scene remains in the $-3$ dB beam-width of the illumination pattern. 
This is typical of radar waveforms and waveforms of opportunity such as
phase shift keying (PSK) modulation found in orthogonal frequency-division multiplexing (OFDM)
common among digital communications. %or typical radar waveforms.
% In active radar, we have control  over the waveform design
% and thus the assumption can be made valid.
% \end{assumption}
% These measurements are
% generally called interferometric measurements and can be modeled as
Using~\eqref{eq:di2}--\eqref{eq:Aij}, the correlated measurements can be modeled as
\begin{equation}
  d_{i,j}(\omega) = \int_{D\times D}
  \mrm{e}^{\mrm{i}\omega/c_0\varphi_{i,j}(\x,\x')}A_{i,j}(\bm{x},\bm{x}', \omega)
  \tilde{\rho}(\bm{x},\bm{x}') d\bm{x} d\bm{x}'\label{eq:dij}
\end{equation}
where
\begin{equation}
  \varphi_{i,j}(\x,\x') = \abs{\x-\a_i^r}+\abs{\x-\a^t}-\abs{\x'-\a_j^r}-\abs{\x'-\a^t},\label{eq:varphi}
\end{equation}
\begin{equation}
  A_{i,j}(\bm{x},\bm{x}', \omega) = A_i(\bm{x}, \omega)A_j^{*}(\bm{x}', \omega)
\end{equation}
and
\begin{equation}
  \tilde{\rho}(\bm{x},\bm{x}') = \rho(\bm{x})\rho^{*}(\bm{x}')
\end{equation}
with $(\cdot)^*$ denoting complex conjugation.
% is the \emph{lifted} reflectivity.
% We will call $\tilde{\rho}$ the \emph{lifted reflectivity}.
We call $\tilde{\rho}$ the lifted version of $\rho$ or the \emph{Kronecker scene}.
% \begin{assumption}\label{assump:farfield}

We next make the small-scene and far-field approximation and approximate the phase term in~\eqref{eq:varphi} % is
% approximated
as
% We assume that $\abs{\a_i^r}\gg \abs{\x}$ for all $\x\in D$ and furthermore, let us assume $J_i =
  % J_j\equiv C$.
% \end{assumption}
% By~\assref{assump:farfield}, we can approximate~\eqref{eq:varphi} as
\begin{equation}
  \varphi_{i,j}(\x,\x') \approx \abs{\a_i^r}-\abs{\a_j^r}-\ip{\hat{\a}_i^r}{\x} + \ip{\hat{\a}_j^r}{\x'}-\ip{\hat{\a}^t}{\x-\x'}\label{eq:varphi2}
\end{equation}
and the amplitude term~\eqref{eq:Aij} as
\begin{equation}
  A_{i,j}(\bm{x},\bm{x}', \omega)\approx \alpha_{i,j}:=\frac{{J_i} (\bm{x}_o \omega) {J_j}(\bm{x}_o, \omega)^*}{\abs{\a_i^r}\abs{\a_j^r}\abs{\a^t}^2}\label{eq:Aij2}
\end{equation}
where $\bm{x}_o$ denotes the center of the scene, and $\hat{\a}$ denotes the unit vector in the direction of $\a$. 
% In other words, we assume that $A_{i,j}$ is approximately independent of spatial variables $\bm{x}$
% and $\bm{x}'$.
% Let $\overline{D}$ be discretization of the domain $\tilde{D}$ such that $\overline{D} = \{\bm{x}_i | i=1,\dots,
% K\}$.
% Then~\eqref{eq:dij} becomes
% \begin{equation}
%   d_{i,j}(\omega) = %\frac{1}{\sqrt{M\binom{N}{2}}}
%   \sum_{\bm{x}_k\in\overline{D}}\sum_{\bm{x}_{k'}\in\overline{D}}\mrm{e}^{\mrm{i}\omega/c_0\varphi_{i,j}(\x_k,\x_{k'})}A_{i,j}\abs{\hat{s}(\omega)}^2
%   \tilde{\rho}(\bm{x}_k,\bm{x}_{k'}) := \mathcal{A}_{i,j}[\tilde{\rho}].\label{eq:dij2}
% \end{equation}
% Let us discretize the
We assume that the support of  the scene is discretized into $K$ discrete spatial points,
$\{\bm{x}_k|\ k=1,\dots,K\}$ and define $\bm{\rho} = [\rho(\bm{x}_1),\dots,\rho(\bm{x}_K)]^T$.
We further assume that the support of $\omega$ is discretized into $M$ samples, $\Omega =
\{\omega_m| m=1,\dots, M\}$
%is discretization of frequency
%space
so that $\bm{d}_{i,j} = [d_{i,j}(\omega_1),\dots,d_{i,j}(\omega_M)]^T$,
$\omega_m = \omega_c - B/2 + \frac{m-1}{M}B$.
% We assume that $B$ is
% the bandwidth and $\omega_c$ is the center frequency so that $\Omega\subset \omega_c+[-B/2,B/2]$.
% Thus,

% Now, let, $\bm{\rho} = \{\rho_k|k=1,...,K\}$ be the discretized reflectivity.
% Then $\tilde{\bm{\rho}} =
% \bm{\rho}\bm{\rho}^T$ is the discretized Kronecker scene.
We write~\eqref{eq:dij} as
\begin{equation}
  d_{i,j}(\omega_m) = %\frac{1}{\sqrt{M\binom{N}{2}}}
  \ip{\L_{i}^m}{\bm{\rho}}\ip{\L_j^m}{\bm{\rho}}^{*} = \opn{tr}\left(\L_j^m(\L_i^m)^H\tilde{\bm{\rho}}\right)\label{eq:dij3}
\end{equation}
where
\begin{equation}
  \L_i^m = [\mrm{e}^{-\mrm{i}\omega_m/c_0 \phi_i(\x_k)}A_i]_{k=1}^K, \qquad i=1,... N.\label{eq:Li}
\end{equation}

Let
% \begin{equation}
%   \bm{d}_{i,j} = [d_{i,j}(\omega_1),\dots, d_{i,j}(\omega_M)]^T
% \end{equation}
% be the vectorized interferometric data for $i,j$ receiver pair.  Then, we denote by
\begin{equation}
  \d = \frac{1}{\sqrt{M\binom{N}{2}}}[\bm{d}_{1,2}^T,\dots, \bm{d}_{N-1,N}^T]^T
\end{equation}
be the full vectorized data scaled by the number of correlated measurements.~\eqref{eq:dij3}
shows that the data vector $\d$ is linear in $\tilde{\bm{\rho}}$,
the  Kronecker scene, while it is non-linear in $\bm{\rho}$.
Thus, the data vector can be written as
\begin{equation}
  \d = \mathcal{F}(\tilde{\bm{\rho}})\label{eq:datamodel}
\end{equation}
where $\mathcal{F}$ is a linear mapping from $\mathbb{R}^{K\times K}$ to $\mathbb{C}^{M\binom{N}{2}}$.
Alternatively, if $\overline{\bm{\rho}}$
is the column-wise vectorization of $\tilde{\bm{\rho}}$, %then the data vector can alternatively be written as
\begin{equation}
  \d = \F\overline{\bm{\rho}}
\end{equation}
where $\F$ is a complex-valued matrix of size $M\binom{N}{2}\times K^2$, whose rows are formed by row-wise
vectorization of the matrix $\L_i^m(\L_j^m)^H$.
